Dynamic Fee for Reducing Impermanent Loss in Decentralized Exchanges

Decentralized exchanges (DEXs) are crucial to decentralized finance (DeFi) as they enable trading without intermediaries. However, they face challenges like impermanent loss (IL), where liquidity providers (LPs) see their assets' value change unfavorably within a liquidity pool compared to outside it. To tackle these issues, we propose dynamic fee mechanisms over traditional fixed-fee structures used in automated market makers (AMM). Our solution includes asymmetric fees via block-adaptive, deal-adaptive, and the "ideal but unattainable" oracle-based fee algorithm, utilizing all data available to arbitrageurs to mitigate IL. We developed a simulation-based framework to compare these fee algorithms systematically. This framework replicates trading on a DEX, considering both informed and uninformed users and a psychological relative loss factor. Results show that adaptive algorithms outperform fixed-fee baselines in reducing IL while maintaining trading activity among uninformed users. Additionally, insights from oracle-based performance underscore the potential of dynamic fee strategies to lower IL, boost LP profitability, and enhance overall market efficiency.

==> historical_data_results.tex <==
\begin{table*}[p]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\textbf{period\_alias} & \textbf{experiment\_name} & \textbf{iu\_markout} & \textbf{iu\_trade\_count} & \textbf{uu\_markout} & \textbf{uu\_trade\_count} & \textbf{lp\_markout} & \textbf{IL
% impermanent\_loss
} \\ \hline
\multirow{4}{*}{\textbf{volatile}} 
 & fixed\_fee                                       & 883900   & 7421 & -314528 & 21415 & -713551    & $2.14664 \times 10^6$ \\ \cline{2-8}
 & based\_on\_trade\_count\_fee                    & 889301   & 7547 & -317706 & 21493 & -716795    & $2.1508 \times 10^6$  \\ \cline{2-8}
 & adaptive\_based\_on\_previous\_block\_price\_move\_fee & 878088 & 7320 & -319057 & 21421 & -702735    & $2.14025 \times 10^6$ \\ \cline{2-8}
 & discrete\_fee\_perfect\_oracle                  & 745471   & 5563 & -318141 & 21426 & -562275    & $1.9954 \times 10^6$  \\ \hline
\hline
\multirow{4}{*}{\textbf{calm}} 
 & fixed\_fee                                       & 21547.3  & 1388 & -222801 & 21478 & 86924.1    & -129736                \\ \cline{2-8}
 & based\_on\_trade\_count\_fee                    & 21597.2  & 1397 & -223315 & 21491 & 87277.4    & -130265                \\ \cline{2-8}
 & adaptive\_based\_on\_previous\_block\_price\_move\_fee & 21556.8 & 1449 & -222936 & 21510 & 86584.1    & -130465                \\ \cline{2-8}
 & discrete\_fee\_perfect\_oracle                  & 17768    & 1016 & -223127 & 21453 & 93014.2    & -135422                \\ \hline
\hline
\multirow{4}{*}{\textbf{bull}} 
 & fixed\_fee                                       & 183885   & 4459 & -272720 & 20864 & -37780.2   & -497942                \\ \cline{2-8}
 & based\_on\_trade\_count\_fee                    & 185121   & 4541 & -270378 & 20759 & -41243.3   & -492462                \\ \cline{2-8}
 & adaptive\_based\_on\_previous\_block\_price\_move\_fee & 180639  & 4392 & -269788 & 20782 & -36720.9   & -505210                \\ \cline{2-8}
 & discrete\_fee\_perfect\_oracle                  & 148360   & 3243 & -271359 & 20813 & 2719.73    & -541723                \\ \hline
\hline
\multirow{4}{*}{\textbf{bear}} 
 & fixed\_fee                                       & 63221.8  & 2199 & -221017 & 20718 & 43210.1    & -183518                \\ \cline{2-8}
 & based\_on\_trade\_count\_fee                    & 63063.2  & 2204 & -222934 & 20858 & 44561.1    & -183516                \\ \cline{2-8}
 & adaptive\_based\_on\_previous\_block\_price\_move\_fee & 63081.5 & 2208 & -222168 & 20784 & 44126.3    & -181757                \\ \cline{2-8}
 & discrete\_fee\_perfect\_oracle                  & 53033.1  & 1538 & -222757 & 20756 & 58253.7    & -192818                \\ \hline
\end{tabular}%
}
\caption{Performance metrics for real-data tests}
\label{tab:grouped_table}
\end{table*}
